Azimuthal harmonics in small and large collision systems at RHIC top energies

The first ($v_1^{\text{even}}$), second ($v_2$) and third ($v_3$) harmonic coefficients of the azimuthal particle distribution at mid-rapidity, are extracted for charged hadrons and studied as a function of transverse momentum ($p_T$) and mean charged particle multiplicity density $\langle \mathrm{N_{ch}} \rangle$ in U+U ($\roots =193$~GeV), Au+Au, Cu+Au, Cu+Cu, $d$+Au and $p$+Au collisions at $\roots = 200$~GeV with the STAR Detector. For the same $\langle \mathrm{N_{ch}} \rangle$, the $v_1^{\text{even}}$ and $v_3$ coefficients are observed to be independent of collision system, while $v_2$ exhibits such a scaling only when normalized by the initial-state eccentricity ($\varepsilon_2$). The data also show that $\ln(v_2/\varepsilon_2)$ scales linearly with $\langle \mathrm{N_{ch}} \rangle^{-1/3}$. These measurements provide insight into initial-geometry fluctuations and the role of viscous hydrodynamic attenuation on $v_n$ from small to large collision systems.

==> authorlist_01242018.tex <==
\author{
J.~Adam$^{12}$,
L.~Adamczyk$^{2}$,
J.~R.~Adams$^{34}$,
J.~K.~Adkins$^{25}$,
G.~Agakishiev$^{23}$,
M.~M.~Aggarwal$^{36}$,
Z.~Ahammed$^{56}$,
I.~Alekseev$^{3,30}$,
D.~M.~Anderson$^{50}$,
R.~Aoyama$^{53}$,
A.~Aparin$^{23}$,
D.~Arkhipkin$^{5}$,
E.~C.~Aschenauer$^{5}$,
M.~U.~Ashraf$^{52}$,
F.~Atetalla$^{24}$,
A.~Attri$^{36}$,
G.~S.~Averichev$^{23}$,
X.~Bai$^{10}$,
V.~Bairathi$^{31}$,
K.~Barish$^{9}$,
A.~J.~Bassill$^{9}$,
A.~Behera$^{48}$,
R.~Bellwied$^{19}$,
A.~Bhasin$^{22}$,
A.~K.~Bhati$^{36}$,
J.~Bielcik$^{13}$,
J.~Bielcikova$^{33}$,
L.~C.~Bland$^{5}$,
I.~G.~Bordyuzhin$^{3}$,
J.~D.~Brandenburg$^{5}$,
A.~V.~Brandin$^{30}$,
D.~Brown$^{27}$,
J.~Bryslawskyj$^{9}$,
I.~Bunzarov$^{23}$,
J.~Butterworth$^{41}$,
H.~Caines$^{59}$,
M.~Calder{\'o}n~de~la~Barca~S{\'a}nchez$^{7}$,
D.~Cebra$^{7}$,
I.~Chakaberia$^{24,45}$,
P.~Chaloupka$^{13}$,
B.~K.~Chan$^{8}$,
F-H.~Chang$^{32}$,
Z.~Chang$^{5}$,
N.~Chankova-Bunzarova$^{23}$,
A.~Chatterjee$^{56}$,
S.~Chattopadhyay$^{56}$,
J.~H.~Chen$^{46}$,
X.~Chen$^{44}$,
J.~Cheng$^{52}$,
M.~Cherney$^{12}$,
W.~Christie$^{5}$,
G.~Contin$^{26}$,
H.~J.~Crawford$^{6}$,
M.~Csanad$^{15}$,
S.~Das$^{10}$,
T.~G.~Dedovich$^{23}$,
I.~M.~Deppner$^{18}$,
A.~A.~Derevschikov$^{38}$,
L.~Didenko$^{5}$,
C.~Dilks$^{37}$,
X.~Dong$^{26}$,
J.~L.~Drachenberg$^{1}$,
J.~C.~Dunlop$^{5}$,
T.~Edmonds$^{39}$,
L.~G.~Efimov$^{23}$,
N.~Elsey$^{58}$,
J.~Engelage$^{6}$,
G.~Eppley$^{41}$,
R.~Esha$^{8}$,
S.~Esumi$^{53}$,
O.~Evdokimov$^{11}$,
J.~Ewigleben$^{27}$,
O.~Eyser$^{5}$,
R.~Fatemi$^{25}$,
S.~Fazio$^{5}$,
P.~Federic$^{33}$,
J.~Fedorisin$^{23}$,
P.~Filip$^{23}$,
E.~Finch$^{47}$,
Y.~Fisyak$^{5}$,
C.~E.~Flores$^{7}$,
L.~Fulek$^{2}$,
C.~A.~Gagliardi$^{50}$,
T.~Galatyuk$^{14}$,
F.~Geurts$^{41}$,
A.~Gibson$^{55}$,
D.~Grosnick$^{55}$,
D.~S.~Gunarathne$^{49}$,
Y.~Guo$^{24}$,
A.~Gupta$^{22}$,
W.~Guryn$^{5}$,
A.~I.~Hamad$^{24}$,
A.~Hamed$^{50}$,
A.~Harlenderova$^{13}$,
J.~W.~Harris$^{59}$,
L.~He$^{39}$,
S.~Heppelmann$^{7}$,
S.~Heppelmann$^{37}$,
N.~Herrmann$^{18}$,
A.~Hirsch$^{39}$,
L.~Holub$^{13}$,
Y.~Hong$^{26}$,
S.~Horvat$^{59}$,
B.~Huang$^{11}$,
H.~Z.~Huang$^{8}$,
S.~L.~Huang$^{48}$,
T.~Huang$^{32}$,
X.~ Huang$^{52}$,
T.~J.~Humanic$^{34}$,
P.~Huo$^{48}$,
G.~Igo$^{8}$,
W.~W.~Jacobs$^{20}$,
A.~Jentsch$^{51}$,
J.~Jia$^{5,48}$,
K.~Jiang$^{44}$,
S.~Jowzaee$^{58}$,
X.~Ju$^{44}$,
E.~G.~Judd$^{6}$,
S.~Kabana$^{24}$,
S.~Kagamaster$^{27}$,
D.~Kalinkin$^{20}$,
K.~Kang$^{52}$,
D.~Kapukchyan$^{9}$,
K.~Kauder$^{5}$,
H.~W.~Ke$^{5}$,
D.~Keane$^{24}$,
A.~Kechechyan$^{23}$,
M.~Kelsey$^{26}$,
D.~P.~Kiko$\l{}$a~$^{57}$,
C.~Kim$^{9}$,
T.~A.~Kinghorn$^{7}$,
I.~Kisel$^{16}$,
A.~Kisiel$^{57}$,
M.~Kocan$^{13}$,
L.~Kochenda$^{30}$,
L.~K.~Kosarzewski$^{13}$,
A.~F.~Kraishan$^{49}$,
L.~Kramarik$^{13}$,
L.~Krauth$^{9}$,
P.~Kravtsov$^{30}$,
K.~Krueger$^{4}$,
N.~Kulathunga$^{19}$,
L.~Kumar$^{36}$,
R.~Kunnawalkam~Elayavalli$^{58}$,
J.~Kvapil$^{13}$,
J.~H.~Kwasizur$^{20}$,
R.~Lacey$^{48}$,
J.~M.~Landgraf$^{5}$,
J.~Lauret$^{5}$,
A.~Lebedev$^{5}$,
R.~Lednicky$^{23}$,
J.~H.~Lee$^{5}$,
C.~Li$^{44}$,
W.~Li$^{46}$,
X.~Li$^{44}$,
Y.~Li$^{52}$,
Y.~Liang$^{24}$,
R.~Licenik$^{13}$,
J.~Lidrych$^{13}$,
T.~Lin$^{50}$,
A.~Lipiec$^{57}$,
M.~A.~Lisa$^{34}$,
F.~Liu$^{10}$,
H.~Liu$^{20}$,
P.~ Liu$^{48}$,
P.~Liu$^{46}$,
X.~Liu$^{34}$,
Y.~Liu$^{50}$,
Z.~Liu$^{44}$,
T.~Ljubicic$^{5}$,
W.~J.~Llope$^{58}$,
M.~Lomnitz$^{26}$,
R.~S.~Longacre$^{5}$,
S.~Luo$^{11}$,
X.~Luo$^{10}$,
G.~L.~Ma$^{46}$,
L.~Ma$^{17}$,
R.~Ma$^{5}$,
Y.~G.~Ma$^{46}$,
N.~Magdy$^{48}$,
R.~Majka$^{59}$,
D.~Mallick$^{31}$,
S.~Margetis$^{24}$,
C.~Markert$^{51}$,
H.~S.~Matis$^{26}$,
O.~Matonoha$^{13}$,
J.~A.~Mazer$^{42}$,
K.~Meehan$^{7}$,
J.~C.~Mei$^{45}$,
N.~G.~Minaev$^{38}$,
S.~Mioduszewski$^{50}$,
D.~Mishra$^{31}$,
B.~Mohanty$^{31}$,
M.~M.~Mondal$^{21}$,
I.~Mooney$^{58}$,
Z.~Moravcova$^{13}$,
D.~A.~Morozov$^{38}$,
Md.~Nasim$^{8}$,
K.~Nayak$^{10}$,
J.~D.~Negrete$^{9}$,
J.~M.~Nelson$^{6}$,
D.~B.~Nemes$^{59}$,
M.~Nie$^{46}$,
G.~Nigmatkulov$^{30}$,
T.~Niida$^{58}$,
L.~V.~Nogach$^{38}$,
T.~Nonaka$^{10}$,
G.~Odyniec$^{26}$,
A.~Ogawa$^{5}$,
K.~Oh$^{40}$,
S.~Oh$^{59}$,
V.~A.~Okorokov$^{30}$,
D.~Olvitt~Jr.$^{49}$,
B.~S.~Page$^{5}$,
R.~Pak$^{5}$,
Y.~Panebratsev$^{23}$,
B.~Pawlik$^{35}$,
H.~Pei$^{10}$,
C.~Perkins$^{6}$,
R.~L.~Pinter$^{15}$,
J.~Pluta$^{57}$,
J.~Porter$^{26}$,
M.~Posik$^{49}$,
N.~K.~Pruthi$^{36}$,
M.~Przybycien$^{2}$,
J.~Putschke$^{58}$,
A.~Quintero$^{49}$,
S.~K.~Radhakrishnan$^{26}$,
R.~L.~Ray$^{51}$,
R.~Reed$^{27}$,
H.~G.~Ritter$^{26}$,
J.~B.~Roberts$^{41}$,
O.~V.~Rogachevskiy$^{23}$,
J.~L.~Romero$^{7}$,
L.~Ruan$^{5}$,
J.~Rusnak$^{33}$,
O.~Rusnakova$^{13}$,
N.~R.~Sahoo$^{50}$,
P.~K.~Sahu$^{21}$,
S.~Salur$^{42}$,
J.~Sandweiss$^{59}$,
J.~Schambach$^{51}$,
A.~M.~Schmah$^{26}$,
W.~B.~Schmidke$^{5}$,
N.~Schmitz$^{28}$,
B.~R.~Schweid$^{48}$,
F.~Seck$^{14}$,
J.~Seger$^{12}$,
M.~Sergeeva$^{8}$,
R.~ Seto$^{9}$,
P.~Seyboth$^{28}$,
N.~Shah$^{46}$,
E.~Shahaliev$^{23}$,
P.~V.~Shanmuganathan$^{27}$,
M.~Shao$^{44}$,
F.~Shen$^{45}$,
W.~Q.~Shen$^{46}$,
S.~S.~Shi$^{10}$,
Q.~Y.~Shou$^{46}$,
E.~P.~Sichtermann$^{26}$,
S.~Siejka$^{57}$,
R.~Sikora$^{2}$,
M.~Simko$^{33}$,
JSingh$^{36}$,
S.~Singha$^{24}$,
D.~Smirnov$^{5}$,
N.~Smirnov$^{59}$,
W.~Solyst$^{20}$,
P.~Sorensen$^{5}$,
H.~M.~Spinka$^{4}$,
B.~Srivastava$^{39}$,
T.~D.~S.~Stanislaus$^{55}$,
D.~J.~Stewart$^{59}$,
M.~Strikhanov$^{30}$,
B.~Stringfellow$^{39}$,
A.~A.~P.~Suaide$^{43}$,
T.~Sugiura$^{53}$,
M.~Sumbera$^{33}$,
B.~Summa$^{37}$,
X.~M.~Sun$^{10}$,
Y.~Sun$^{44}$,
B.~Surrow$^{49}$,
D.~N.~Svirida$^{3}$,
P.~Szymanski$^{57}$,
A.~H.~Tang$^{5}$,
Z.~Tang$^{44}$,
A.~Taranenko$^{30}$,
T.~Tarnowsky$^{29}$,
J.~H.~Thomas$^{26}$,
A.~R.~Timmins$^{19}$,
D.~Tlusty$^{41}$,
T.~Todoroki$^{5}$,
M.~Tokarev$^{23}$,
C.~A.~Tomkiel$^{27}$,
S.~Trentalange$^{8}$,
R.~E.~Tribble$^{50}$,
P.~Tribedy$^{5}$,
S.~K.~Tripathy$^{21}$,
O.~D.~Tsai$^{8}$,
B.~Tu$^{10}$,
T.~Ullrich$^{5}$,
D.~G.~Underwood$^{4}$,
I.~Upsal$^{5,45}$,
G.~Van~Buren$^{5}$,
J.~Vanek$^{33}$,
A.~N.~Vasiliev$^{38}$,
I.~Vassiliev$^{16}$,
F.~Videb{\ae}k$^{5}$,
S.~Vokal$^{23}$,
S.~A.~Voloshin$^{58}$,
A.~Vossen$^{20}$,
F.~Wang$^{39}$,
G.~Wang$^{8}$,
P.~Wang$^{44}$,
Y.~Wang$^{10}$,
Y.~Wang$^{52}$,
J.~C.~Webb$^{5}$,
L.~Wen$^{8}$,
G.~D.~Westfall$^{29}$,
H.~Wieman$^{26}$,
S.~W.~Wissink$^{20}$,
R.~Witt$^{54}$,
Y.~Wu$^{24}$,
Z.~G.~Xiao$^{52}$,
G.~Xie$^{11}$,
W.~Xie$^{39}$,
J.~Xu$^{10}$,
N.~Xu$^{26}$,
Q.~H.~Xu$^{45}$,
Y.~F.~Xu$^{46}$,
Z.~Xu$^{5}$,
C.~Yang$^{45}$,
Q.~Yang$^{45}$,
S.~Yang$^{5}$,
Y.~Yang$^{32}$,
Z.~Ye$^{11}$,
Z.~Ye$^{11}$,
L.~Yi$^{45}$,
K.~Yip$^{5}$,
I.~-K.~Yoo$^{40}$,
H.~Zbroszczyk$^{57}$,
W.~Zha$^{44}$,
D.~Zhang$^{10}$,
J.~Zhang$^{48}$,
L.~Zhang$^{10}$,
S.~Zhang$^{44}$,
S.~Zhang$^{46}$,
X.~P.~Zhang$^{52}$,
Y.~Zhang$^{44}$,
Z.~Zhang$^{46}$,
J.~Zhao$^{39}$,
C.~Zhong$^{46}$,
C.~Zhou$^{46}$,
X.~Zhu$^{52}$,
Z.~Zhu$^{45}$,
M.~K.~Zurek$^{26}$,
M.~Zyzak$^{16}$
}
%
\address{$^{1}$Abilene Christian University, Abilene, Texas   79699}
\address{$^{2}$AGH University of Science and Technology, FPACS, Cracow 30-059, Poland}
\address{$^{3}$Alikhanov Institute for Theoretical and Experimental Physics, Moscow 117218, Russia}
\address{$^{4}$Argonne National Laboratory, Argonne, Illinois 60439}
\address{$^{5}$Brookhaven National Laboratory, Upton, New York 11973}
\address{$^{6}$University of California, Berkeley, California 94720}
\address{$^{7}$University of California, Davis, California 95616}
\address{$^{8}$University of California, Los Angeles, California 90095}
\address{$^{9}$University of California, Riverside, California 92521}
\address{$^{10}$Central China Normal University, Wuhan, Hubei 430079 }
\address{$^{11}$University of Illinois at Chicago, Chicago, Illinois 60607}
\address{$^{12}$Creighton University, Omaha, Nebraska 68178}
\address{$^{13}$Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\address{$^{14}$Technische Universit\"at Darmstadt, Darmstadt 64289, Germany}
\address{$^{15}$E\"otv\"os Lor\'and University, Budapest, Hungary H-1117}
\address{$^{16}$Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\address{$^{17}$Fudan University, Shanghai, 200433 }
\address{$^{18}$University of Heidelberg, Heidelberg 69120, Germany }
\address{$^{19}$University of Houston, Houston, Texas 77204}
\address{$^{20}$Indiana University, Bloomington, Indiana 47408}
\address{$^{21}$Institute of Physics, Bhubaneswar 751005, India}
\address{$^{22}$University of Jammu, Jammu 180001, India}
\address{$^{23}$Joint Institute for Nuclear Research, Dubna 141 980, Russia}
\address{$^{24}$Kent State University, Kent, Ohio 44242}
\address{$^{25}$University of Kentucky, Lexington, Kentucky 40506-0055}
\address{$^{26}$Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\address{$^{27}$Lehigh University, Bethlehem, Pennsylvania 18015}
\address{$^{28}$Max-Planck-Institut f\"ur Physik, Munich 80805, Germany}
\address{$^{29}$Michigan State University, East Lansing, Michigan 48824}
\address{$^{30}$National Research Nuclear University MEPhI, Moscow 115409, Russia}
\address{$^{31}$National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\address{$^{32}$National Cheng Kung University, Tainan 70101 }
\address{$^{33}$Nuclear Physics Institute of the CAS, Rez 250 68, Czech Republic}
\address{$^{34}$Ohio State University, Columbus, Ohio 43210}
\address{$^{35}$Institute of Nuclear Physics PAN, Cracow 31-342, Poland}
\address{$^{36}$Panjab University, Chandigarh 160014, India}
\address{$^{37}$Pennsylvania State University, University Park, Pennsylvania 16802}
\address{$^{38}$Institute of High Energy Physics, Protvino 142281, Russia}
\address{$^{39}$Purdue University, West Lafayette, Indiana 47907}
\address{$^{40}$Pusan National University, Pusan 46241, Korea}
\address{$^{41}$Rice University, Houston, Texas 77251}
\address{$^{42}$Rutgers University, Piscataway, New Jersey 08854}
\address{$^{43}$Universidade de S\~ao Paulo, S\~ao Paulo, Brazil 05314-970}
\address{$^{44}$University of Science and Technology of China, Hefei, Anhui 230026}
\address{$^{45}$Shandong University, Qingdao, Shandong 266237}
\address{$^{46}$Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\address{$^{47}$Southern Connecticut State University, New Haven, Connecticut 06515}
\address{$^{48}$State University of New York, Stony Brook, New York 11794}
\address{$^{49}$Temple University, Philadelphia, Pennsylvania 19122}
\address{$^{50}$Texas A\&M University, College Station, Texas 77843}
\address{$^{51}$University of Texas, Austin, Texas 78712}
\address{$^{52}$Tsinghua University, Beijing 100084}
\address{$^{53}$University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\address{$^{54}$United States Naval Academy, Annapolis, Maryland 21402}
\address{$^{55}$Valparaiso University, Valparaiso, Indiana 46383}
\address{$^{56}$Variable Energy Cyclotron Centre, Kolkata 700064, India}
\address{$^{57}$Warsaw University of Technology, Warsaw 00-661, Poland}
\address{$^{58}$Wayne State University, Detroit, Michigan 48201}
\address{$^{59}$Yale University, New Haven, Connecticut 06520}
